CesASMe and Staticdeps: static detection of memory-carried dependencies for code analyzers

A variety of code analyzers, such as IACA, uiCA, llvm-mca or Ithemal, strive to statically predict the throughput of a computation kernel. Each analyzer is based on its own simplified CPU model reasoning at the scale of a basic block. Facing this diversity, evaluating their strengths and weaknesses is important to guide both their usage and their enhancement. We present CesASMe, a fully-tooled solution to evaluate code analyzers on C-level benchmarks composed of a benchmark derivation procedure that feeds an evaluation harness. We conclude that memory-carried data dependencies are a major source of imprecision for these tools. We tackle this issue with staticdeps, a static analyzer extracting memory-carried data dependencies, including across loop iterations, from an assembly basic block. We integrate its output to uiCA, a state-of-the-art code analyzer, to evaluate staticdeps' impact on a code analyzer's precision through CesASMe.

==> 05_related_works.tex <==
\section{Related works}

\todo{Changer l'histoire par rapport à AniCA}

The static throughput analyzers studied rely on a variety of models.
\iaca~\cite{iaca}, developed by Intel and now deprecated, is closed-source and
relies on Intel's expertise on their own processors.
The LLVM compiling ecosystem, to guide optimization passes, maintains models of many
architectures. These models are used in the LLVM Machine Code Analyzer,
\llvmmca~\cite{llvm-mca}, to statically evaluate the performance of a segment
of assembly.
Independently, Abel and Reineke used an automated microbenchmark generation
approach to generate port mappings of many architectures in
\texttt{uops.info}~\cite{nanobench, uopsinfo} to model processors' backends.
This work was continued with \uica~\cite{uica}, extending this model with an
extensive frontend description.
Following a completely different approach, \ithemal~\cite{ithemal} uses a deep
neural network to predict basic blocks throughput. To obtain enough data to
train its model, the authors also developed \bhive~\cite{bhive}, a profiling
tool working on basic blocks.

Another static tool, \osaca~\cite{osaca2}, provides lower- and
upper-bounds to the execution time of a basic block. As this kind of
information cannot be fairly compared with tools yielding an exact throughput
prediction, we exclude it from our scope.

All these tools statically predict the number of cycles taken by a piece of
assembly or binary that is assumed to be the body of an infinite ---~or
sufficiently large~--- loop in steady state, all its data being L1-resident. As
discussed by \uica's authors~\cite{uica}, hypotheses can subtly vary between
analyzers; \eg{} by assuming that the loop is either unrolled or has control
instructions, with non-negligible impact. Some of the tools, \eg{} \ithemal,
necessarily work on a single basic block, while some others, \eg{} \iaca, work
on a section of code delimited by markers. However, even in the second case,
the code is assumed to be \emph{straight-line code}: branch instructions, if
any, are assumed not taken.

\smallskip

Throughput prediction tools, however, are not all static.
\gus~\cite{phd:gruber} dynamically predicts the throughput of a whole program
region, instrumenting it to retrieve the exact events occurring through its
execution. This way, \gus{} can more finely detect bottlenecks by
sensitivity analysis, at the cost of a significantly longer run time.

\smallskip

The \bhive{} profiler~\cite{bhive} takes another approach to basic block
throughput measurement: by mapping memory at any address accessed by a basic
block, it can effectively run and measure arbitrary code without context, often
---~but not always, as we discuss later~--- yielding good results.

\smallskip

The \anica{} framework~\cite{anica} also attempts to evaluate throughput
predictors by finding examples on which they are inaccurate. \anica{} starts
with randomly generated assembly snippets, and refines them through a process
derived from abstract interpretation to reach general categories of problems.


==> 10_bench_gen.tex <==
\section{Generating microbenchmarks}\label{sec:bench_gen}

Our framework aims to generate \emph{microbenchmarks} relevant to a specific
domain.
A microbenchmark is a code that is as simplified as possible to expose the
behaviour under consideration.
The specified computations should be representative of the considered domain,
and at the same time they should stress the different aspects of the
target architecture ---~which is modeled by code analyzers.

In practice, a microbenchmark's \textit{computational kernel} is a simple
\texttt{for} loop, whose
body contains no loops and whose bounds are statically known.
A \emph{measure} is a number of repetitions $n$ of this computational
kernel, $n$ being a user-specified parameter.
The measure may be repeated an arbitrary number of times to improve
stability.

Furthermore, such a microbenchmark should be a function whose computation
happens without leaving the L1 cache.
This requirement helps measurements and analyses to be
undisturbed by memory accesses, but it is also a matter of comparability.
Indeed, most of the static analyzers make the assumption that the code under
consideration is L1-resident; if it is not, their results are meaningless, and
can not be compared with an actual measurement.

The generation of such microbenchmarks is achieved through four distinct
components, whose parameter variations are specified in configuration files~:
a benchmark suite, C-to-C loop nest optimizers, a constraining utility
and a C-to-binary compiler.

\subsection{Benchmark suite}\label{ssec:bench_suite}
Our first component is an initial set of benchmarks which materializes
the human expertise we intend to exploit for the generation of relevant codes.
The considered suite must embed computation kernels
delimited by ad-hoc \texttt{\#pragma}s,
whose arrays are accessed
directly (no indirections) and whose loops are affine.
These constraints are necessary to ensure that the microkernelification phase,
presented below, generates segfault-free code.

In this case, we use Polybench~\cite{polybench}, a suite of 30
benchmarks for polyhedral compilation ---~of which we use only 26. The
\texttt{nussinov}, \texttt{ludcmp} and \texttt{deriche} benchmarks are
removed because they are incompatible with PoCC (introduced below). The
\texttt{lu} benchmark is left out as its execution alone takes longer than all
others together, making its dynamic analysis (\eg{} with \gus) impractical.
In addition to the importance of linear algebra within
it, one of its important features is that it does not include computational
kernels with conditional control flow (\eg{} \texttt{if-then-else})
---~however, it does include conditional data flow, using the ternary
conditional operator of C.

\subsection{C-to-C loop nest optimizers}\label{ssec:loop_nest_optimizer}
Loop nest optimizers transform an initial benchmark in different ways (generate different
\textit{versions} of the same benchmark), varying the stress on
resources of the target architecture, and by extension the models on which the
static analyzers are based.

In this case, we chose to use the
\textsc{Pluto}~\cite{pluto} and PoCC~\cite{pocc} polyhedral compilers, to easily access common loop nest optimizations~: register tiling, tiling,
skewing, vectorization/simdization, loop unrolling, loop permutation,
loop fusion.
These transformations are meant to maximize variety within the initial
benchmark suite. Eventually, the generated benchmarks are expected to
highlight the impact on performance of the resulting behaviours.
For instance, \textit{skewing} introduces non-trivial pointer arithmetic,
increasing the pressure on address computation units; \textit{loop unrolling},
among many things, opens the way to register promotion, which
alleviates load-store units by reducing spilling;
\textit{vectorization} stresses SIMD units and decreases
pressure on the front-end; \textit{loop permutation} may move dependant
instructions apart from each other, lessening latency-induced slowdowns;
and so on.

\subsection{Constraining utility}\label{ssec:kernelify}

A constraining utility transforms the code in order to respect an arbitrary number of non-functional
properties.
In this case, we apply a pass of \emph{microkernelification}: we
extract a computational kernel from the arbitrarily deep and arbitrarily
long loop nest generated by the previous component.
The loop chosen to form the microkernel is the one considered to be
the \textit{hottest}; the \textit{hotness} of a loop being obtained by
multiplying the number of arithmetic operations it contains by the number of
times it is iterated. This metric allows us to prioritize the parts of the
code that have the greatest impact on performance.

At this point, the resulting code can
compute a different result from the initial code;
for instance, the composition of tiling and
kernelification reduces the number of loop iterations.
Indeed, our framework is not meant to preserve the
functional semantics of the benchmarks.
Our goal is only to generate codes that are relevant from the point of view of
performance analysis.

\subsection{C-to-binary compiler}\label{ssec:compile}

A C-to-binary compiler varies binary optimization options by
enabling/disabling auto-vectorization, extended instruction
sets, \textit{etc}. We use \texttt{gcc}.

\bigskip

Eventually, the relevance of the microbenchmarks set generated using this approach
derives not only from initial benchmark suite and the relevance of the
transformations chosen at each
stage, but also from the combinatorial explosion generated by the composition
of the four stages. In our experimental setup, this yields up to 144
microbenchmarks per benchmark of the original suite.


==> 25_results_analysis.tex <==
\section{Results analysis}\label{sec:results_analysis}


==> contrib.tex <==
\section{Contributions}

\subsection{Generation of interesting micro benchs}

Apply high-level and low-level transformations on benchmarks from polybenchs
in order to:
\begin{itemize}
\item Grant the L1-residence (small enough) of the generated
  micro-benchmark.
\item Control different bottlenecks: latency, front-end throughput, ports
  throughputs, registers pressure, ILP...
\item Expose significative differences between analyzers.
\end{itemize}

Difference with AnICA: real-world kernels instead of randomly-generated
code.

\subsubsection{High-level (polyhedral) transformations}

\begin{itemize}
\item Tiling (skewing, no skewing), different tiling configurations, loop
  permutation: adresses computation.
\item Register tiling, different unroll factors: expose registers pressure and
  ILP.
\item Dimensions permutations
\item Fusion
\item ...
\end{itemize}

\subsubsection{Low-level (code generation) transformations}

Control vectorization level:
\begin{itemize}
\item Vectorization or not.
\item AVX, AVX2 or AVX512.
\item ...
\end{itemize}

\subsection{Given a microbench, comparison between measure and multiple code analyzers}

\subsubsection{Static markers make the job impossible}

Iaca markers (used by iaca, uica, ithemal...):
\begin{itemize}
\item Mess with registers, thus a marked code can not be
  executed. Therefore, measure and prediction are performed on different
  binaries and are hardly comparable.
\item May change the compilation flow (they come with memory barriers).
\end{itemize}

Llvm-mca markers are assembly comments, meaning that they can not be handled
with analyzers working on binary-level.

\subsubsection{Real-world kernels vs basic blocks}

If static marks are unavailable, most tools have to consume basic blocks,
and their predictions must be compared to basic block-level measurements
(e.g. Bhive)
It is the approach choosen by AnICA.

Eventually, these predictions can hardly be compared to measurements on
real-world kernels (e.g. under the form of a C function with memory
allocation, conditional branching, for loops...). The data has to be
post-processed (e.g. multiply the duration of a basic block by how many
times it is iterated), but some parameters may be missing (e.g. the unroll
factor applied by the compiler to a particular loop), and even if all the
parameters are available, the measurement is still imprecise.

\subsubsection{Our proposal}

\subsection{Evaluation of Gus}


Pour l'instant il ne faut pas se fier à ce que donne le register tiling :
on doit modifier légèrement l'algorithme d'identification de la hottest loop
(ie le pondérer par le nombre de flops dans la loop), car sans cela la
kernelification évince la boucle déroulée au profit d'une boucle plus banale
(atteinte un plus grand nombre de fois mais réalisant beaucoup moins
d'opérations dans le corps de boucle, donc en toute rigueur moins "hot").

Il est néanmoins possible de faire quelques observations :
- Une erreur significative de Gus prend généralement la forme d'une
surestimation du temps d'exécution, et généralement aussi vient avec une
surestimation considérable des latences (donner le même kernel à gus en
désactivant les latences produit un résultat beaucoup plus proche de la
mesure/des autres analyseurs).
- Dès qu'un kernel est L1-resident (pas de L1 cache misses) ET qu'il n'y a pas
de dépendances entre les tours de boucle, Gus réussit très bien.
- Dès qu'un kernel n'est pas L1-resident et produit un nombre significatif
- Il faut ajouter aux benchs sur lesquels Gus réussit très bien les versions
tilées (en particulier 16x16x16) de atax, bicg et gesummv, alors même que ces
derniers transportent des dépendances d'un tour de boucle à l'autre. Tous
trois sont de la forme $X[c4]=X[c4]+Y[c4][c3]*Z[c3]$

